Compressibility of Distributed Document Representations

Contemporary natural language processing (NLP) revolves around learning from latent document representations, generated either implicitly by neural language models or explicitly by methods such as doc2vec or similar. One of the key properties of the obtained representations is their dimension. Whilst the commonly adopted dimensions of 256 and 768 offer sufficient performance on many tasks, it is many times unclear whether the default dimension is the most suitable choice for the subsequent downstream learning tasks. Furthermore, representation dimensions are seldom subject to hyperparameter tuning due to computational constraints. The purpose of this paper is to demonstrate that a surprisingly simple and efficient recursive compression procedure can be sufficient to both significantly compress the initial representation, but also potentially improve its performance when considering the task of text classification. Having smaller and less noisy representations is the desired property during deployment, as orders of magnitude smaller models can significantly reduce the computational overload and with it the deployment costs. We propose CoRe, a straightforward, representation learner-agnostic framework suitable for representation compression. The CoRe's performance is showcased and studied on a collection of 17 real-life corpora from biomedical, news, social media, and literary domains. We explored CoRe's behavior when considering contextual and non-contextual document representations, different compression levels, and 9 different compression algorithms. Current results based on more than 100,000 compression experiments indicate that recursive Singular Value Decomposition offers a very good trade-off between the compression efficiency and performance, making CoRe useful in many existing, representation-dependent NLP pipelines.

==> datasets.tex <==
\begin{tabular}{lcccc}
\toprule
                   Data set &  Documents &  Tokens &  Max length &  Unique labels \\
\midrule
 %    semeval-2017 &       1156 &    4929 &                   21 &              4 \\
                        bbc &       1406 &   49418 &                  343 &              4 \\
                   subjects &       1786 &  104972 &                  227 &              4 \\
                   CNN-news &       2107 &  144077 &                  605 &              7 \\
            pan-2017 &       3599 &  575670 &                 1478 &              2 \\
                    insults &       3946 &   29133 &                  288 &              2 \\
                  questions &       5452 &   13278 &                   37 &              6 \\
                    SMSSpam &       5571 &   17744 &                   88 &              2 \\
            MedRelation &       8361 &   16796 &                   99 &              2 \\
 AAAI2021 &       8473 &   41387 &                  149 &              2 \\
                       mbti &       8675 &  313038 &                  419 &             16 \\
                       yelp &      10000 &   76482 &                  592 &              5 \\
                 hatespeech &      10557 &   29982 &                  195 &              4 \\
                semeval-2019 &      13240 &   39714 &                  155 &              2 \\
                   articles &      19990 &  285144 &                10692 &             20 \\
                    sarcasm &      28619 &   50241 &                  166 &              2 \\
                    authors &      53678 &   29997 &                 1008 &             45 \\
            drugs-condition &      70406 &   96879 &                  435 &            150 \\
\bottomrule
\end{tabular}


==> table_BERT_CoRe-large-dir.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
            mbti &               9 (dim = 2) &       0.002305 \\
         insults &               7 (dim = 6) &      -0.038501 \\
    pan-2017-age &               7 (dim = 6) &       0.128713 \\
         SMSSpam &              6 (dim = 12) &      -0.033070 \\
            yelp &              5 (dim = 24) &      -0.012800 \\
          kenyan &             2 (dim = 192) &      -0.034483 \\
        CNN-news &             1 (dim = 384) &      -0.045541 \\
        articles &             1 (dim = 384) &      -0.049420 \\
 MedicalRelation &             0 (dim = 768) &       0.000000 \\
         authors &             0 (dim = 768) &       0.000000 \\
 drugs-condition &             0 (dim = 768) &       0.000000 \\
       questions &             0 (dim = 768) &       0.000000 \\
         sarcasm &             0 (dim = 768) &       0.000000 \\
\bottomrule
\end{tabular}


==> table_BERT_CoRe-large-rec.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
            mbti &               9 (dim = 2) &       0.002305 \\
         insults &               7 (dim = 6) &      -0.041540 \\
    pan-2017-age &               7 (dim = 6) &       0.089109 \\
         SMSSpam &              6 (dim = 12) &      -0.039540 \\
            yelp &              6 (dim = 12) &      -0.038800 \\
        CNN-news &             2 (dim = 192) &      -0.045541 \\
          kenyan &             2 (dim = 192) &      -0.043103 \\
 MedicalRelation &             1 (dim = 384) &      -0.047824 \\
        articles &             1 (dim = 384) &      -0.044218 \\
         authors &             0 (dim = 768) &       0.000000 \\
 drugs-condition &             0 (dim = 768) &       0.000000 \\
       questions &             0 (dim = 768) &       0.000000 \\
         sarcasm &             0 (dim = 768) &       0.000000 \\
\bottomrule
\end{tabular}


==> table_BERT_CoRe-small-dir.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         insults &               9 (dim = 2) &      -0.041540 \\
            mbti &               9 (dim = 2) &       0.002766 \\
         SMSSpam &               7 (dim = 6) &      -0.030913 \\
    pan-2017-age &               7 (dim = 6) &       0.128713 \\
            yelp &               7 (dim = 6) &      -0.019600 \\
        CNN-news &              3 (dim = 96) &      -0.045541 \\
        articles &              3 (dim = 96) &      -0.043617 \\
 MedicalRelation &             2 (dim = 192) &      -0.036346 \\
          kenyan &             2 (dim = 192) &      -0.034483 \\
       questions &             2 (dim = 192) &      -0.049156 \\
         sarcasm &             2 (dim = 192) &      -0.040391 \\
         authors &             1 (dim = 384) &      -0.036513 \\
 drugs-condition &             1 (dim = 384) &      -0.033455 \\
\bottomrule
\end{tabular}


==> table_BERT_CoRe-small-rec.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
            mbti &               9 (dim = 2) &       0.000922 \\
    pan-2017-age &               7 (dim = 6) &       0.089109 \\
         SMSSpam &              6 (dim = 12) &      -0.026600 \\
         insults &              6 (dim = 12) &      -0.013171 \\
            yelp &              6 (dim = 12) &      -0.020400 \\
        CNN-news &              3 (dim = 96) &      -0.036053 \\
        articles &              3 (dim = 96) &      -0.044018 \\
 MedicalRelation &             2 (dim = 192) &      -0.043998 \\
          kenyan &             2 (dim = 192) &      -0.017241 \\
       questions &             2 (dim = 192) &      -0.046222 \\
         sarcasm &             2 (dim = 192) &      -0.043606 \\
         authors &             1 (dim = 384) &      -0.035618 \\
 drugs-condition &             1 (dim = 384) &      -0.032659 \\
\bottomrule
\end{tabular}


==> table_BERT_PCA-dir.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         insults &               9 (dim = 2) &      -0.042553 \\
            mbti &               9 (dim = 2) &       0.002305 \\
         SMSSpam &               7 (dim = 6) &      -0.040259 \\
    pan-2017-age &               7 (dim = 6) &       0.089109 \\
            yelp &               7 (dim = 6) &      -0.026800 \\
        CNN-news &              3 (dim = 96) &      -0.037951 \\
        articles &              3 (dim = 96) &      -0.046819 \\
          kenyan &              3 (dim = 96) &      -0.034483 \\
 MedicalRelation &             2 (dim = 192) &      -0.047824 \\
       questions &             2 (dim = 192) &      -0.044754 \\
         sarcasm &             2 (dim = 192) &      -0.042907 \\
         authors &             1 (dim = 384) &      -0.029732 \\
 drugs-condition &             1 (dim = 384) &      -0.023969 \\
\bottomrule
\end{tabular}


==> table_BERT_PCA.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         insults &               9 (dim = 2) &      -0.042553 \\
            mbti &               9 (dim = 2) &       0.002766 \\
         SMSSpam &               7 (dim = 6) &      -0.040259 \\
    pan-2017-age &               7 (dim = 6) &       0.089109 \\
            yelp &               7 (dim = 6) &      -0.025600 \\
        CNN-news &              3 (dim = 96) &      -0.045541 \\
        articles &              3 (dim = 96) &      -0.047219 \\
          kenyan &              3 (dim = 96) &      -0.034483 \\
 MedicalRelation &             2 (dim = 192) &      -0.043998 \\
       questions &             2 (dim = 192) &      -0.048423 \\
         sarcasm &             2 (dim = 192) &      -0.040391 \\
         authors &             1 (dim = 384) &      -0.029583 \\
 drugs-condition &             1 (dim = 384) &      -0.025957 \\
\bottomrule
\end{tabular}


==> table_BERT_SVD.tex <==
\begin{tabular}{llr}
\toprule
                    Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
                       yelp &                 9 (dim = 2) &      -0.086000 \\
                    sarcasm &                 9 (dim = 2) &      -0.302586 \\
                    SMSSpam &                 9 (dim = 2) &      -0.073329 \\
                   SentiMix &                 9 (dim = 2) &      -0.081176 \\
     semeval-2017-sentiment &                 9 (dim = 2) &      -0.013841 \\
                   articles &                 9 (dim = 2) &      -0.589936 \\
                  questions &                 9 (dim = 2) &      -0.405723 \\
                   CNN-news &                 9 (dim = 2) &      -0.574953 \\
                    authors &                 9 (dim = 2) &      -0.297876 \\
                        bbc &                 9 (dim = 2) &      -0.420455 \\
            counterfactuals &                 9 (dim = 2) &      -0.052000 \\
            MedicalRelation &                 9 (dim = 2) &      -0.322334 \\
                    insults &                 9 (dim = 2) &      -0.042553 \\
                   subjects &                 9 (dim = 2) &      -0.194631 \\
 AAAI2021-COVID19-fake-news &                 9 (dim = 2) &      -0.207477 \\
                       mbti &                 9 (dim = 2) &       0.005533 \\
                 hatespeech &                 9 (dim = 2) &      -0.005848 \\
                semeval2019 &                 9 (dim = 2) &      -0.084290 \\
                   subjects &                 8 (dim = 3) &      -0.109620 \\
                   SentiMix &                 8 (dim = 3) &      -0.051294 \\
                       mbti &                 8 (dim = 3) &       0.007838 \\
                   articles &                 8 (dim = 3) &      -0.531613 \\
                    sarcasm &                 8 (dim = 3) &      -0.279525 \\
     semeval-2017-sentiment &                 8 (dim = 3) &       0.000000 \\
                    authors &                 8 (dim = 3) &      -0.298435 \\
                    insults &                 8 (dim = 3) &      -0.031408 \\
                        bbc &                 8 (dim = 3) &      -0.215909 \\
                    SMSSpam &                 8 (dim = 3) &      -0.058231 \\
                 hatespeech &                 8 (dim = 3) &      -0.007310 \\
            counterfactuals &                 8 (dim = 3) &      -0.052000 \\
                  questions &                 8 (dim = 3) &      -0.424065 \\
                   CNN-news &                 8 (dim = 3) &      -0.535104 \\
            MedicalRelation &                 8 (dim = 3) &      -0.157819 \\
                       yelp &                 8 (dim = 3) &      -0.052800 \\
                semeval2019 &                 8 (dim = 3) &      -0.073414 \\
 AAAI2021-COVID19-fake-news &                 8 (dim = 3) &      -0.201402 \\
                   subjects &                 7 (dim = 6) &      -0.069351 \\
                    sarcasm &                 7 (dim = 6) &      -0.239693 \\
                        bbc &                 7 (dim = 6) &      -0.119318 \\
                       mbti &                 7 (dim = 6) &       0.008760 \\
                       yelp &                 7 (dim = 6) &      -0.023600 \\
            counterfactuals &                 7 (dim = 6) &      -0.052000 \\
            MedicalRelation &                 7 (dim = 6) &      -0.138211 \\
                   SentiMix &                 7 (dim = 6) &      -0.047529 \\
     semeval-2017-sentiment &                 7 (dim = 6) &      -0.015571 \\
                    authors &                 7 (dim = 6) &      -0.280812 \\
                semeval2019 &                 7 (dim = 6) &      -0.057402 \\
                   articles &                 7 (dim = 6) &      -0.458683 \\
 AAAI2021-COVID19-fake-news &                 7 (dim = 6) &      -0.099065 \\
                    SMSSpam &                 7 (dim = 6) &      -0.039540 \\
                    insults &                 7 (dim = 6) &      -0.020263 \\
                 hatespeech &                 7 (dim = 6) &      -0.008041 \\
                   CNN-news &                 7 (dim = 6) &      -0.324478 \\
                  questions &                 7 (dim = 6) &      -0.333822 \\
                    insults &                6 (dim = 12) &      -0.020263 \\
                       mbti &                6 (dim = 12) &       0.020286 \\
                   CNN-news &                6 (dim = 12) &      -0.234345 \\
                    authors &                6 (dim = 12) &      -0.241654 \\
     semeval-2017-sentiment &                6 (dim = 12) &      -0.012111 \\
 AAAI2021-COVID19-fake-news &                6 (dim = 12) &      -0.069626 \\
                 hatespeech &                6 (dim = 12) &      -0.005665 \\
                        bbc &                6 (dim = 12) &      -0.056818 \\
                semeval2019 &                6 (dim = 12) &      -0.039577 \\
                    sarcasm &                6 (dim = 12) &      -0.163103 \\
                   articles &                6 (dim = 12) &      -0.322729 \\
            counterfactuals &                6 (dim = 12) &      -0.052923 \\
            MedicalRelation &                6 (dim = 12) &      -0.140603 \\
                   SentiMix &                6 (dim = 12) &      -0.031294 \\
                   subjects &                6 (dim = 12) &      -0.026846 \\
                       yelp &                6 (dim = 12) &      -0.002800 \\
                    SMSSpam &                6 (dim = 12) &      -0.025881 \\
                  questions &                6 (dim = 12) &      -0.254585 \\
                    insults &                5 (dim = 24) &      -0.010132 \\
                    sarcasm &                5 (dim = 24) &      -0.130119 \\
            counterfactuals &                5 (dim = 24) &      -0.035692 \\
                   CNN-news &                5 (dim = 24) &      -0.148008 \\
                semeval2019 &                5 (dim = 24) &      -0.020846 \\
 AAAI2021-COVID19-fake-news &                5 (dim = 24) &      -0.054206 \\
                        bbc &                5 (dim = 24) &      -0.019886 \\
            MedicalRelation &                5 (dim = 24) &      -0.134385 \\
                    SMSSpam &                5 (dim = 24) &      -0.025162 \\
                       yelp &                5 (dim = 24) &       0.006400 \\
                  questions &                5 (dim = 24) &      -0.209831 \\
                   SentiMix &                5 (dim = 24) &      -0.027765 \\
     semeval-2017-sentiment &                5 (dim = 24) &       0.006920 \\
                   subjects &                5 (dim = 24) &      -0.017897 \\
                   articles &                5 (dim = 24) &      -0.195178 \\
                       mbti &                5 (dim = 24) &       0.016598 \\
                    authors &                5 (dim = 24) &      -0.212146 \\
                 hatespeech &                5 (dim = 24) &       0.003655 \\
 AAAI2021-COVID19-fake-news &                4 (dim = 48) &      -0.038318 \\
                       mbti &                4 (dim = 48) &       0.020747 \\
                   subjects &                4 (dim = 48) &      -0.013423 \\
                  questions &                4 (dim = 48) &      -0.159941 \\
                    insults &                4 (dim = 48) &      -0.009119 \\
                    sarcasm &                4 (dim = 48) &      -0.108316 \\
                    authors &                4 (dim = 48) &      -0.166356 \\
                 hatespeech &                4 (dim = 48) &       0.010599 \\
            MedicalRelation &                4 (dim = 48) &      -0.105691 \\
                       yelp &                4 (dim = 48) &       0.018400 \\
     semeval-2017-sentiment &                4 (dim = 48) &       0.013841 \\
                   SentiMix &                4 (dim = 48) &      -0.023059 \\
                        bbc &                4 (dim = 48) &      -0.008523 \\
                semeval2019 &                4 (dim = 48) &      -0.016918 \\
                   articles &                4 (dim = 48) &      -0.092637 \\
                    SMSSpam &                4 (dim = 48) &      -0.009346 \\
            counterfactuals &                4 (dim = 48) &      -0.025231 \\
                   CNN-news &                4 (dim = 48) &      -0.080645 \\
                  questions &                3 (dim = 96) &      -0.110785 \\
                semeval2019 &                3 (dim = 96) &       0.003625 \\
 AAAI2021-COVID19-fake-news &                3 (dim = 96) &      -0.017290 \\
                    SMSSpam &                3 (dim = 96) &      -0.000719 \\
                   articles &                3 (dim = 96) &      -0.048519 \\
                   SentiMix &                3 (dim = 96) &      -0.014118 \\
                       mbti &                3 (dim = 96) &       0.025357 \\
            MedicalRelation &                3 (dim = 96) &      -0.090387 \\
                 hatespeech &                3 (dim = 96) &       0.011696 \\
                    sarcasm &                3 (dim = 96) &      -0.072816 \\
                       yelp &                3 (dim = 96) &       0.020000 \\
                    authors &                3 (dim = 96) &      -0.110768 \\
                        bbc &                3 (dim = 96) &       0.000000 \\
                   subjects &                3 (dim = 96) &       0.002237 \\
                    insults &                3 (dim = 96) &       0.005066 \\
            counterfactuals &                3 (dim = 96) &      -0.010462 \\
                   CNN-news &                3 (dim = 96) &      -0.039848 \\
     semeval-2017-sentiment &                3 (dim = 96) &      -0.003460 \\
                    sarcasm &               2 (dim = 192) &      -0.038854 \\
     semeval-2017-sentiment &               2 (dim = 192) &      -0.013841 \\
                semeval2019 &               2 (dim = 192) &       0.013293 \\
                   subjects &               2 (dim = 192) &       0.000000 \\
                  questions &               2 (dim = 192) &      -0.049890 \\
            counterfactuals &               2 (dim = 192) &      -0.010462 \\
 AAAI2021-COVID19-fake-news &               2 (dim = 192) &      -0.007477 \\
                   CNN-news &               2 (dim = 192) &      -0.020873 \\
            MedicalRelation &               2 (dim = 192) &      -0.036346 \\
                    SMSSpam &               2 (dim = 192) &       0.000719 \\
                   SentiMix &               2 (dim = 192) &       0.006824 \\
                   articles &               2 (dim = 192) &      -0.029612 \\
                    authors &               2 (dim = 192) &      -0.064158 \\
                        bbc &               2 (dim = 192) &       0.002841 \\
                       yelp &               2 (dim = 192) &       0.024800 \\
                       mbti &               2 (dim = 192) &       0.011987 \\
                 hatespeech &               2 (dim = 192) &       0.009137 \\
                    insults &               2 (dim = 192) &       0.013171 \\
     semeval-2017-sentiment &               1 (dim = 384) &      -0.003460 \\
                   SentiMix &               1 (dim = 384) &      -0.001882 \\
                   subjects &               1 (dim = 384) &       0.000000 \\
                  questions &               1 (dim = 384) &      -0.022010 \\
                   CNN-news &               1 (dim = 384) &      -0.003795 \\
            MedicalRelation &               1 (dim = 384) &      -0.003348 \\
                       mbti &               1 (dim = 384) &       0.003688 \\
                    SMSSpam &               1 (dim = 384) &       0.000719 \\
                    insults &               1 (dim = 384) &       0.002026 \\
 AAAI2021-COVID19-fake-news &               1 (dim = 384) &      -0.000467 \\
                semeval2019 &               1 (dim = 384) &       0.005740 \\
                   articles &               1 (dim = 384) &      -0.018507 \\
                    authors &               1 (dim = 384) &      -0.028353 \\
                    sarcasm &               1 (dim = 384) &      -0.018588 \\
                        bbc &               1 (dim = 384) &       0.000000 \\
                 hatespeech &               1 (dim = 384) &       0.012792 \\
                       yelp &               1 (dim = 384) &       0.021200 \\
            counterfactuals &               1 (dim = 384) &      -0.004923 \\
                       yelp &               0 (dim = 768) &       0.000000 \\
 AAAI2021-COVID19-fake-news &               0 (dim = 768) &       0.000000 \\
                   subjects &               0 (dim = 768) &       0.000000 \\
                semeval2019 &               0 (dim = 768) &       0.000000 \\
     semeval-2017-sentiment &               0 (dim = 768) &       0.000000 \\
                    sarcasm &               0 (dim = 768) &       0.000000 \\
                  questions &               0 (dim = 768) &       0.000000 \\
                       mbti &               0 (dim = 768) &       0.000000 \\
                    insults &               0 (dim = 768) &       0.000000 \\
            counterfactuals &               0 (dim = 768) &       0.000000 \\
                        bbc &               0 (dim = 768) &       0.000000 \\
                    authors &               0 (dim = 768) &       0.000000 \\
                   articles &               0 (dim = 768) &       0.000000 \\
                   SentiMix &               0 (dim = 768) &       0.000000 \\
                    SMSSpam &               0 (dim = 768) &       0.000000 \\
            MedicalRelation &               0 (dim = 768) &       0.000000 \\
                   CNN-news &               0 (dim = 768) &       0.000000 \\
                 hatespeech &               0 (dim = 768) &       0.000000 \\
\bottomrule
\end{tabular}


==> table_BERT_UMAP-dir.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         SMSSpam &               9 (dim = 2) &      -0.036664 \\
         insults &               9 (dim = 2) &      -0.037487 \\
            mbti &               9 (dim = 2) &       0.002305 \\
    pan-2017-age &               7 (dim = 6) &       0.039604 \\
            yelp &              6 (dim = 12) &      -0.033600 \\
        CNN-news &             0 (dim = 768) &       0.000000 \\
 MedicalRelation &             0 (dim = 768) &       0.000000 \\
        articles &             0 (dim = 768) &       0.000000 \\
         authors &             0 (dim = 768) &       0.000000 \\
 drugs-condition &             0 (dim = 768) &       0.000000 \\
          kenyan &             0 (dim = 768) &       0.000000 \\
       questions &             0 (dim = 768) &       0.000000 \\
         sarcasm &             0 (dim = 768) &       0.000000 \\
\bottomrule
\end{tabular}


==> table_BERT_UMAP.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
            mbti &               9 (dim = 2) &       0.002305 \\
    pan-2017-age &               7 (dim = 6) &       0.049505 \\
         SMSSpam &              3 (dim = 96) &      -0.030194 \\
         insults &             1 (dim = 384) &      -0.033435 \\
            yelp &             1 (dim = 384) &      -0.034800 \\
        CNN-news &             0 (dim = 768) &       0.000000 \\
 MedicalRelation &             0 (dim = 768) &       0.000000 \\
        articles &             0 (dim = 768) &       0.000000 \\
         authors &             0 (dim = 768) &       0.000000 \\
 drugs-condition &             0 (dim = 768) &       0.000000 \\
          kenyan &             0 (dim = 768) &       0.000000 \\
       questions &             0 (dim = 768) &       0.000000 \\
         sarcasm &             0 (dim = 768) &       0.000000 \\
\bottomrule
\end{tabular}


==> table_doc2vec_CoRe-large-dir.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         insults &               9 (dim = 2) &      -0.020263 \\
         SMSSpam &               7 (dim = 6) &      -0.046010 \\
    pan-2017-age &               7 (dim = 6) &       0.079208 \\
        CNN-news &              6 (dim = 12) &       0.011385 \\
            yelp &              6 (dim = 12) &      -0.038400 \\
          kenyan &              5 (dim = 24) &      -0.008621 \\
       questions &              5 (dim = 24) &      -0.035950 \\
         sarcasm &              5 (dim = 24) &      -0.044864 \\
 MedicalRelation &              4 (dim = 48) &      -0.023912 \\
        articles &              4 (dim = 48) &      -0.035214 \\
            mbti &              4 (dim = 48) &       0.064085 \\
         authors &              3 (dim = 96) &      -0.036215 \\
 drugs-condition &             1 (dim = 384) &      -0.036238 \\
\bottomrule
\end{tabular}


==> table_doc2vec_CoRe-large-rec.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         insults &               9 (dim = 2) &      -0.014184 \\
    pan-2017-age &               7 (dim = 6) &       0.059406 \\
       questions &              6 (dim = 12) &       0.000734 \\
        CNN-news &              5 (dim = 24) &       0.039848 \\
         SMSSpam &              5 (dim = 24) &      -0.038821 \\
 MedicalRelation &              4 (dim = 48) &      -0.016260 \\
            mbti &              4 (dim = 48) &       0.012448 \\
         sarcasm &              4 (dim = 48) &      -0.028092 \\
            yelp &              4 (dim = 48) &      -0.036400 \\
        articles &              3 (dim = 96) &      -0.025010 \\
         authors &              3 (dim = 96) &      -0.040238 \\
          kenyan &              3 (dim = 96) &      -0.034483 \\
 drugs-condition &             1 (dim = 384) &      -0.034022 \\
\bottomrule
\end{tabular}


==> table_doc2vec_CoRe-small-dir.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         insults &               9 (dim = 2) &      -0.017224 \\
         SMSSpam &               8 (dim = 3) &      -0.023005 \\
        CNN-news &               7 (dim = 6) &       0.032258 \\
    pan-2017-age &               7 (dim = 6) &       0.099010 \\
            yelp &               7 (dim = 6) &      -0.020800 \\
       questions &              6 (dim = 12) &      -0.046955 \\
         sarcasm &              6 (dim = 12) &      -0.041509 \\
 MedicalRelation &              5 (dim = 24) &      -0.043042 \\
        articles &              5 (dim = 24) &      -0.045018 \\
          kenyan &              5 (dim = 24) &      -0.043103 \\
            mbti &              5 (dim = 24) &       0.061319 \\
         authors &              4 (dim = 48) &      -0.046870 \\
 drugs-condition &             2 (dim = 192) &      -0.040100 \\
\bottomrule
\end{tabular}


==> table_doc2vec_CoRe-small-rec.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         insults &               9 (dim = 2) &      -0.018237 \\
    pan-2017-age &               7 (dim = 6) &       0.059406 \\
       questions &               7 (dim = 6) &      -0.024945 \\
         SMSSpam &              6 (dim = 12) &      -0.023724 \\
        CNN-news &              5 (dim = 24) &       0.018975 \\
         sarcasm &              5 (dim = 24) &      -0.049755 \\
 MedicalRelation &              4 (dim = 48) &      -0.032520 \\
            mbti &              4 (dim = 48) &       0.002766 \\
            yelp &              4 (dim = 48) &      -0.023200 \\
        articles &              3 (dim = 96) &      -0.040216 \\
          kenyan &              3 (dim = 96) &      -0.008621 \\
 drugs-condition &             2 (dim = 192) &      -0.042770 \\
         authors &             1 (dim = 384) &      -0.020790 \\
\bottomrule
\end{tabular}


==> table_doc2vec_PCA-dir.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         insults &               9 (dim = 2) &      -0.022290 \\
         SMSSpam &               8 (dim = 3) &      -0.028037 \\
        CNN-news &               7 (dim = 6) &      -0.005693 \\
    pan-2017-age &               7 (dim = 6) &      -0.009901 \\
       questions &               7 (dim = 6) &      -0.044754 \\
          kenyan &              6 (dim = 12) &      -0.043103 \\
         sarcasm &              6 (dim = 12) &      -0.039413 \\
            yelp &              6 (dim = 12) &      -0.034800 \\
 MedicalRelation &              5 (dim = 24) &      -0.041129 \\
        articles &              5 (dim = 24) &      -0.043818 \\
            mbti &              5 (dim = 24) &       0.032273 \\
         authors &              3 (dim = 96) &      -0.021311 \\
 drugs-condition &             2 (dim = 192) &      -0.033171 \\
\bottomrule
\end{tabular}


==> table_doc2vec_PCA.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         SMSSpam &               9 (dim = 2) &      -0.036664 \\
         insults &               9 (dim = 2) &      -0.026342 \\
        CNN-news &               7 (dim = 6) &       0.005693 \\
    pan-2017-age &               7 (dim = 6) &       0.019802 \\
       questions &               7 (dim = 6) &      -0.026412 \\
         sarcasm &              6 (dim = 12) &      -0.040391 \\
            yelp &              6 (dim = 12) &      -0.026400 \\
 MedicalRelation &              5 (dim = 24) &      -0.047346 \\
        articles &              5 (dim = 24) &      -0.044218 \\
          kenyan &              5 (dim = 24) &      -0.043103 \\
            mbti &              5 (dim = 24) &       0.028124 \\
         authors &              4 (dim = 48) &      -0.049478 \\
 drugs-condition &             2 (dim = 192) &      -0.033625 \\
\bottomrule
\end{tabular}


==> table_doc2vec_SVD.tex <==
\begin{tabular}{llr}
\toprule
                    Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
                       yelp &                 9 (dim = 2) &  -1.177000e-01 \\
            pan-2017-gender &                 9 (dim = 2) &  -1.801587e-01 \\
                       mbti &                 9 (dim = 2) &  -2.303234e-01 \\
            MedicalRelation &                 9 (dim = 2) &  -1.747967e-01 \\
                   SentiMix &                 9 (dim = 2) &  -1.494118e-01 \\
     semeval-2017-sentiment &                 9 (dim = 2) &   0.000000e+00 \\
                   articles &                 9 (dim = 2) &  -5.311553e-01 \\
                  questions &                 9 (dim = 2) &  -2.079971e-01 \\
                   CNN-news &                 9 (dim = 2) &  -3.667661e-01 \\
                    authors &                 9 (dim = 2) &  -7.566000e-01 \\
                    insults &                 9 (dim = 2) &  -2.077001e-02 \\
                        bbc &                 9 (dim = 2) &  -2.913961e-01 \\
                    SMSSpam &                 9 (dim = 2) &  -6.593407e-02 \\
                    sarcasm &                 9 (dim = 2) &  -2.066287e-01 \\
                semeval2019 &                 9 (dim = 2) &  -4.350453e-02 \\
            drugs-condition &                 9 (dim = 2) &  -3.616056e-01 \\
 AAAI2021-COVID19-fake-news &                 9 (dim = 2) &  -4.626168e-02 \\
            counterfactuals &                 9 (dim = 2) &   5.846154e-03 \\
                   subjects &                 9 (dim = 2) &  -8.948546e-02 \\
                 hatespeech &                 9 (dim = 2) &   3.715887e-03 \\
                   articles &                 8 (dim = 3) &  -4.274281e-01 \\
                       mbti &                 8 (dim = 3) &  -2.143845e-01 \\
                   SentiMix &                 8 (dim = 3) &  -1.497143e-01 \\
            drugs-condition &                 8 (dim = 3) &  -3.171971e-01 \\
                 hatespeech &                 8 (dim = 3) &   4.203216e-03 \\
                  questions &                 8 (dim = 3) &  -1.261005e-01 \\
                    sarcasm &                 8 (dim = 3) &  -1.647000e-01 \\
                   subjects &                 8 (dim = 3) &  -8.501119e-02 \\
                    authors &                 8 (dim = 3) &  -6.571535e-01 \\
            counterfactuals &                 8 (dim = 3) &   5.846154e-03 \\
                    SMSSpam &                 8 (dim = 3) &  -3.306973e-02 \\
                        bbc &                 8 (dim = 3) &  -7.142857e-02 \\
                    insults &                 8 (dim = 3) &  -1.671733e-02 \\
     semeval-2017-sentiment &                 8 (dim = 3) &   0.000000e+00 \\
                   CNN-news &                 8 (dim = 3) &  -1.976145e-01 \\
 AAAI2021-COVID19-fake-news &                 8 (dim = 3) &  -4.372497e-02 \\
                       yelp &                 8 (dim = 3) &  -1.140000e-01 \\
            MedicalRelation &                 8 (dim = 3) &  -1.713893e-01 \\
                semeval2019 &                 8 (dim = 3) &  -4.350453e-02 \\
            pan-2017-gender &                 8 (dim = 3) &  -1.846032e-01 \\
                        bbc &                 7 (dim = 6) &  -1.014610e-02 \\
     semeval-2017-sentiment &                 7 (dim = 6) &   0.000000e+00 \\
                    authors &                 7 (dim = 6) &  -5.178199e-01 \\
                       yelp &                 7 (dim = 6) &  -4.860000e-02 \\
                   CNN-news &                 7 (dim = 6) &  -1.057197e-02 \\
                    insults &                 7 (dim = 6) &  -1.963019e-02 \\
                semeval2019 &                 7 (dim = 6) &  -4.333189e-02 \\
                   articles &                 7 (dim = 6) &  -2.572458e-01 \\
            counterfactuals &                 7 (dim = 6) &   5.142857e-03 \\
 AAAI2021-COVID19-fake-news &                 7 (dim = 6) &  -4.105474e-02 \\
                    sarcasm &                 7 (dim = 6) &  -1.251273e-01 \\
            drugs-condition &                 7 (dim = 6) &  -2.563250e-01 \\
                 hatespeech &                 7 (dim = 6) &   1.157407e-03 \\
            pan-2017-gender &                 7 (dim = 6) &  -4.603175e-03 \\
                  questions &                 7 (dim = 6) &  -6.438004e-02 \\
            MedicalRelation &                 7 (dim = 6) &  -1.753945e-01 \\
                   subjects &                 7 (dim = 6) &  -3.515500e-02 \\
                       mbti &                 7 (dim = 6) &  -1.483896e-01 \\
                    SMSSpam &                 7 (dim = 6) &  -1.478895e-02 \\
                   SentiMix &                 7 (dim = 6) &  -5.361345e-02 \\
                   CNN-news &                6 (dim = 12) &   3.957712e-02 \\
                       yelp &                6 (dim = 12) &  -2.120000e-02 \\
                  questions &                6 (dim = 12) &  -2.173514e-02 \\
                    sarcasm &                6 (dim = 12) &  -4.284716e-02 \\
                   articles &                6 (dim = 12) &  -1.481450e-01 \\
 AAAI2021-COVID19-fake-news &                6 (dim = 12) &  -3.591455e-02 \\
                   SentiMix &                6 (dim = 12) &  -3.213445e-02 \\
                        bbc &                6 (dim = 12) &  -5.275974e-03 \\
                    insults &                6 (dim = 12) &  -1.393110e-02 \\
            counterfactuals &                6 (dim = 12) &   2.637363e-04 \\
                   subjects &                6 (dim = 12) &  -2.524768e-02 \\
            pan-2017-gender &                6 (dim = 12) &   3.095238e-02 \\
            drugs-condition &                6 (dim = 12) &  -1.982684e-01 \\
                       mbti &                6 (dim = 12) &  -9.102285e-02 \\
            MedicalRelation &                6 (dim = 12) &  -9.803922e-02 \\
                 hatespeech &                6 (dim = 12) &  -9.746589e-04 \\
                    authors &                6 (dim = 12) &  -3.408026e-01 \\
                semeval2019 &                6 (dim = 12) &  -4.285714e-02 \\
                    SMSSpam &                6 (dim = 12) &  -5.648557e-03 \\
     semeval-2017-sentiment &                6 (dim = 12) &   0.000000e+00 \\
                       yelp &                5 (dim = 24) &   1.200000e-03 \\
            drugs-condition &                5 (dim = 24) &  -1.623229e-01 \\
                    sarcasm &                5 (dim = 24) &  -3.274433e-02 \\
                  questions &                5 (dim = 24) &  -5.777696e-03 \\
            pan-2017-gender &                5 (dim = 24) &   2.238095e-02 \\
 AAAI2021-COVID19-fake-news &                5 (dim = 24) &  -2.309746e-02 \\
                   articles &                5 (dim = 24) &  -5.162065e-02 \\
                   SentiMix &                5 (dim = 24) &  -1.129412e-02 \\
            counterfactuals &                5 (dim = 24) &  -6.945055e-03 \\
                   subjects &                5 (dim = 24) &  -5.752637e-03 \\
                    insults &                5 (dim = 24) &  -9.118541e-03 \\
                   CNN-news &                5 (dim = 24) &   4.418542e-02 \\
                        bbc &                5 (dim = 24) &  -7.711039e-03 \\
     semeval-2017-sentiment &                5 (dim = 24) &   0.000000e+00 \\
                    SMSSpam &                5 (dim = 24) &   6.162062e-04 \\
                    authors &                5 (dim = 24) &  -1.661167e-01 \\
                semeval2019 &                5 (dim = 24) &  -4.190764e-02 \\
                       mbti &                5 (dim = 24) &   6.355793e-02 \\
            MedicalRelation &                5 (dim = 24) &  -4.752511e-02 \\
                 hatespeech &                5 (dim = 24) &   2.253899e-03 \\
            pan-2017-gender &                4 (dim = 48) &   3.936508e-02 \\
                    insults &                4 (dim = 48) &   6.332320e-04 \\
                 hatespeech &                4 (dim = 48) &   4.264133e-04 \\
                       mbti &                4 (dim = 48) &   1.200685e-01 \\
     semeval-2017-sentiment &                4 (dim = 48) &   0.000000e+00 \\
                   articles &                4 (dim = 48) &  -1.812153e-02 \\
                        bbc &                4 (dim = 48) &  -1.298701e-02 \\
 AAAI2021-COVID19-fake-news &                4 (dim = 48) &  -1.769025e-02 \\
                   CNN-news &                4 (dim = 48) &   4.662510e-02 \\
            MedicalRelation &                4 (dim = 48) &  -2.702056e-02 \\
                semeval2019 &                4 (dim = 48) &  -3.059991e-02 \\
                    SMSSpam &                4 (dim = 48) &   7.189073e-04 \\
                   SentiMix &                4 (dim = 48) &  -6.890756e-03 \\
                       yelp &                4 (dim = 48) &   7.000000e-04 \\
                    authors &                4 (dim = 48) &  -4.941452e-02 \\
                  questions &                4 (dim = 48) &  -1.650770e-03 \\
                    sarcasm &                4 (dim = 48) &  -1.808925e-02 \\
                   subjects &                4 (dim = 48) &  -7.350591e-03 \\
            drugs-condition &                4 (dim = 48) &  -1.281544e-01 \\
            counterfactuals &                4 (dim = 48) &  -5.494505e-03 \\
                   subjects &                3 (dim = 96) &  -7.350591e-03 \\
                        bbc &                3 (dim = 96) &  -1.298701e-02 \\
 AAAI2021-COVID19-fake-news &                3 (dim = 96) &  -6.208278e-03 \\
                   CNN-news &                3 (dim = 96) &   1.870426e-02 \\
            MedicalRelation &                3 (dim = 96) &  -1.464610e-02 \\
            drugs-condition &                3 (dim = 96) &  -8.814365e-02 \\
                semeval2019 &                3 (dim = 96) &  -8.718170e-03 \\
            pan-2017-gender &                3 (dim = 96) &   4.285714e-02 \\
                    SMSSpam &                3 (dim = 96) &   7.189073e-04 \\
                 hatespeech &                3 (dim = 96) &   1.827485e-03 \\
                   SentiMix &                3 (dim = 96) &   3.361345e-04 \\
            counterfactuals &                3 (dim = 96) &  -2.329670e-03 \\
                    insults &                3 (dim = 96) &   1.773050e-03 \\
                   articles &                3 (dim = 96) &  -6.145315e-03 \\
                    sarcasm &                3 (dim = 96) &  -5.730259e-03 \\
                       mbti &                3 (dim = 96) &   1.375222e-01 \\
                       yelp &                3 (dim = 96) &   8.600000e-03 \\
                    authors &                3 (dim = 96) &  -1.973600e-02 \\
                  questions &                3 (dim = 96) &  -1.467351e-03 \\
     semeval-2017-sentiment &                3 (dim = 96) &   0.000000e+00 \\
                semeval2019 &               2 (dim = 192) &  -5.179111e-04 \\
                    sarcasm &               2 (dim = 192) &  -1.118099e-03 \\
     semeval-2017-sentiment &               2 (dim = 192) &   0.000000e+00 \\
                   subjects &               2 (dim = 192) &  -4.154682e-03 \\
                  questions &               2 (dim = 192) &  -1.283933e-03 \\
            MedicalRelation &               2 (dim = 192) &  -9.026781e-03 \\
                       yelp &               2 (dim = 192) &  -7.000000e-04 \\
                   articles &               2 (dim = 192) &  -6.002401e-04 \\
                        bbc &               2 (dim = 192) &  -4.870130e-03 \\
                   SentiMix &               2 (dim = 192) &   4.302521e-03 \\
            counterfactuals &               2 (dim = 192) &   2.681319e-03 \\
                    SMSSpam &               2 (dim = 192) &   6.162062e-04 \\
            drugs-condition &               2 (dim = 192) &  -3.855017e-02 \\
                    authors &               2 (dim = 192) &  -1.865020e-02 \\
                 hatespeech &               2 (dim = 192) &   1.827485e-03 \\
                   CNN-news &               2 (dim = 192) &   2.168609e-03 \\
                    insults &               2 (dim = 192) &   2.026342e-03 \\
                       mbti &               2 (dim = 192) &   1.323849e-01 \\
 AAAI2021-COVID19-fake-news &               2 (dim = 192) &  -3.471295e-03 \\
            pan-2017-gender &               2 (dim = 192) &   3.222222e-02 \\
                    authors &               1 (dim = 384) &  -1.214605e-02 \\
            MedicalRelation &               1 (dim = 384) &  -8.548541e-03 \\
                   SentiMix &               1 (dim = 384) &   4.672269e-03 \\
                semeval2019 &               1 (dim = 384) &  -3.452741e-04 \\
                   CNN-news &               1 (dim = 384) &  -2.710762e-04 \\
                   articles &               1 (dim = 384) &  -1.180472e-02 \\
                    SMSSpam &               1 (dim = 384) &   6.162062e-04 \\
                       yelp &               1 (dim = 384) &   1.300000e-03 \\
                        bbc &               1 (dim = 384) &  -4.464286e-03 \\
                  questions &               1 (dim = 384) &  -1.283933e-03 \\
     semeval-2017-sentiment &               1 (dim = 384) &   0.000000e+00 \\
            counterfactuals &               1 (dim = 384) &   2.637363e-03 \\
                   subjects &               1 (dim = 384) &  -3.835091e-03 \\
            drugs-condition &               1 (dim = 384) &  -1.136788e-02 \\
 AAAI2021-COVID19-fake-news &               1 (dim = 384) &  -3.337784e-03 \\
                 hatespeech &               1 (dim = 384) &   1.827485e-03 \\
                    insults &               1 (dim = 384) &   2.026342e-03 \\
                    sarcasm &               1 (dim = 384) &  -7.587102e-04 \\
                       mbti &               1 (dim = 384) &   8.028716e-02 \\
            pan-2017-gender &               1 (dim = 384) &   1.619048e-02 \\
                       yelp &               0 (dim = 768) &   2.800000e-03 \\
 AAAI2021-COVID19-fake-news &               0 (dim = 768) &  -3.404539e-03 \\
                   subjects &               0 (dim = 768) &  -3.835091e-03 \\
                semeval2019 &               0 (dim = 768) &  -3.884333e-04 \\
                   CNN-news &               0 (dim = 768) &  -1.586033e-17 \\
            MedicalRelation &               0 (dim = 768) &  -8.548541e-03 \\
                    SMSSpam &               0 (dim = 768) &   6.162062e-04 \\
                   SentiMix &               0 (dim = 768) &   4.705882e-03 \\
                   articles &               0 (dim = 768) &  -4.230264e-03 \\
                    authors &               0 (dim = 768) &   1.681925e-03 \\
                        bbc &               0 (dim = 768) &  -4.464286e-03 \\
            counterfactuals &               0 (dim = 768) &   2.637363e-03 \\
            drugs-condition &               0 (dim = 768) &   5.030753e-04 \\
                    insults &               0 (dim = 768) &   2.026342e-03 \\
                       mbti &               0 (dim = 768) &   2.219588e-02 \\
            pan-2017-gender &               0 (dim = 768) &  -7.936508e-04 \\
                  questions &               0 (dim = 768) &  -1.375642e-03 \\
                    sarcasm &               0 (dim = 768) &  -6.588799e-04 \\
     semeval-2017-sentiment &               0 (dim = 768) &   0.000000e+00 \\
                 hatespeech &               0 (dim = 768) &   1.827485e-03 \\
\bottomrule
\end{tabular}


==> table_doc2vec_UMAP-dir.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         SMSSpam &               9 (dim = 2) &       0.000000 \\
         insults &               8 (dim = 3) &      -0.021277 \\
    pan-2017-age &               7 (dim = 6) &       0.009901 \\
       questions &               7 (dim = 6) &      -0.026412 \\
 MedicalRelation &              4 (dim = 48) &      -0.042563 \\
        CNN-news &             0 (dim = 768) &       0.000000 \\
        articles &             0 (dim = 768) &       0.000000 \\
         authors &             0 (dim = 768) &       0.000000 \\
 drugs-condition &             0 (dim = 768) &       0.000000 \\
          kenyan &             0 (dim = 768) &       0.000000 \\
            mbti &             0 (dim = 768) &       0.000000 \\
         sarcasm &             0 (dim = 768) &       0.000000 \\
            yelp &             0 (dim = 768) &       0.000000 \\
\bottomrule
\end{tabular}


==> table_doc2vec_UMAP.tex <==
\begin{tabular}{llr}
\toprule
         Dataset & Compression step ($\kappa$) &  $\epsilon F1$ \\
\midrule
         insults &               9 (dim = 2) &      -0.018237 \\
    pan-2017-age &               7 (dim = 6) &       0.089109 \\
         SMSSpam &              3 (dim = 96) &      -0.000719 \\
       questions &              3 (dim = 96) &      -0.005869 \\
 MedicalRelation &             2 (dim = 192) &      -0.021043 \\
        CNN-news &             0 (dim = 768) &       0.000000 \\
        articles &             0 (dim = 768) &       0.000000 \\
         authors &             0 (dim = 768) &       0.000000 \\
 drugs-condition &             0 (dim = 768) &       0.000000 \\
          kenyan &             0 (dim = 768) &       0.000000 \\
            mbti &             0 (dim = 768) &       0.000000 \\
         sarcasm &             0 (dim = 768) &       0.000000 \\
            yelp &             0 (dim = 768) &       0.000000 \\
\bottomrule
\end{tabular}

